Blockchain-based Data Provenance for the Internet of Things

As more and more applications and services depend on data collected and provided by Internet of Things (IoT) devices, it is of importance that such data can be trusted. Data provenance solutions together with blockchain technology are one way to make data more trustworthy. However, current solutions do not address the heterogeneous nature of IoT applications and their data. In this work, we identify functional and non-functional requirements for a generic IoT data provenance framework, and conceptualise the framework as a layered architecture. Using a proof-of-concept implementation based on Ethereum smart contracts, data provenance can be realised for a wide range of IoT use cases. Benefits of a generic framework include simplified adoption and a more rapid implementation of data provenance for the IoT.

==> sections/04implementation.tex <==
\section{Implementation}
\label{sec:implementation}
This section presents a proof-of-concept implementation of the framework based on Ethereum smart contracts. The smart contracts are written in Solidity and are available as open-source software\footnote{\url{https://github.com/iotprovenance/iotprovenance}}.

\subsection{Provenance Storage Contract}
As described in \cref{sec:storage-layer}, the storage layer of the framework provides low-level storage functionality of provenance records. Some of the internals of the smart contract implementing this layer are shown in \cref{lst:provenance-records}. The data structure for a provenance record contains the fields defined by the provenance data model described in~\cref{sec:provenance-model}, such as input provenance IDs and the context. To recall, the context needs to contain all information necessary for a concrete provenance use case. The current prototype implements the context parameter as string value to allow storing any kind of information. To save storage costs, \textit{context} could hold a hash which references provenance data stored in a content-addressable storage such as IPFS\footnote{\url{https://ipfs.io/}}. The \textit{tokenId} field references the data point for which the provenance record was created. 

The contract stores provenance records as a mapping $\textit{addr}(\textit{prov}) \mapsto \textit{prov}$. The mapping is implemented via the \textit{mapping} keyword~(Line 8). As mentioned in~\cref{sec:architecture}, this mapping enables random access by the ID of a data point. Further, the contract defines a field \textit{provenanceIndex} implemented as an array containing all provenance IDs within the system~(Line~9). These IDs can be used for iteration over provenance records. The contract exposes an API for creating, retrieving, updating, and deleting (i.e., invalidating) provenance records. Note that, while functionality for retrieving provenance records is exposed publicly via the \textit{public} keyword, functionality for creating, updating, and deleting records is protected via the \textit{internal} keyword. These functions cannot be accessed publicly, but are accessible from inheriting contracts such as the contract representing the generic provenance layer. Read-functions are publicly accessible since these functions do not alter the state of the contract.

%\begin{lstlisting}[caption={Mapping from IDs to Provenance Records}, label=lst:mapping-example, float]
%mapping (uint => ProvenanceRecord) private records;
%\end{lstlisting}

\begin{lstlisting}[caption={Storage Contract}, label=lst:provenance-records, float]
contract Storage {
struct ProvenanceRecord {
    uint tokenId;
    uint[] inputProvenanceIds;
    string context;
    uint index;
}
mapping (uint -> ProvenanceRecord) records;
uint[] provenanceIndex;

function getProvenance(uint provId)
public view returns (uint tokenId, ...) {...}
...
function createProvenance(uint provId, ...) 
internal returns (uint index) {...}
...
}
\end{lstlisting}

\subsection{Generic Provenance Contract}
As mentioned above, the generic provenance layer augments the storage layer by generic provenance functionality. The contract implementing this layer is primarily responsible for managing the ownership of data points and associating data points to their respective provenance records. As described in \cref{sec:generic-provenance-layer}, our framework uses tokens to represent data points. Consequently, ownership of tokens determines ownership of data points. Data points represent non-fungible assets. As such, the contract implements the Ethereum standard ERC721 which defines a common interface for non-fungible assets, for instance, functions for transferring ownership. This has the advantage that our tokens can be traded by any clients implementing this standard, such as wallets or exchanges. The generic provenance contract complies to the standard by inheriting from an existing ERC721 implementation provided by OpenZeppelin\footnote{\url{https://openzeppelin.org/}}.

\Cref{lst:associated-provenance} displays an outline of the contract and demonstrates the general workflow for creating new provenance records. First, the contract verifies that a given token (i.e., data point) exists~(Line~7) and that the token belongs to the sender of the message~(Line~8). After validating the input provenance records~(Line~9), the contract creates a new provenance ID~(Line~11), adds it to the list of associated provenance~(Line~12), and calls the storage contract's \textit{createProvenance} function~(Line~13). Note that the \textit{createProvenance} function of the generic contract is again internal, and can thus not be accessed publicly. This enables specific provenance contracts which implement concrete use cases to further adapt the functionality according to their needs. 

\begin{lstlisting}[caption={Generic Provenance Contract}, label={lst:associated-provenance}, float]
contract GenericProvenance is ERC721, Storage {
...
mapping (uint => uint[]) internal associatedProv;
...
function createProvenance(uint tokenId, ...) 
internal returns (uint index) {
    require(exists(tokenId));
    require(ownerOf(tokenId) == msg.sender);
    checkValidProvenance(inputProvenance);

    uint provId = getProvId();
    addAssociatedProvenance(tokenId, provId);
    return super.createProvenance(provId, ...);
}
...
\end{lstlisting}

\subsection{Specific Provenance Contracts}
\label{sec:implementation-specific}
As briefly mentioned in \cref{sec:specific-provenance-layer}, the contracts of the specific provenance layer adapt the behaviour provided by the generic provenance layer to reflect the requirements of specific provenance use cases, i.e., by customising the provenance model, and by certain access control mechanisms. 

The provenance model can be customised by defining the contents of the \textit{context} parameter, so that it presents the provenance information needed for a specific provenance scenario. For instance, in the use case of vaccine supply chains (see Section~\ref{sec:usecase1}), the context should contain temperature and location information about individual vaccines. Hence, a specific contract could define its own \textit{createProvenance} function that requires parameters like \textit{temperature}, and \textit{location} which are then combined to form the \textit{context} to be passed on to the \textit{createProvenance} function of the generic provenance contract.

Further, access control happens on two levels. First, a specific contract defines which parts of the generic provenance layer's API are exposed. For instance, even though the generic provenance layer permits updating or deleting (i.e., invalidating) provenance records, this can be unwanted behaviour in the specific use case at hand. In this case, the contract in the specific provenance layer implementing the use case  simply ``hides'' the functionality, i.e., does not expose it publicly.

Second, access control is relevant for controlling the ownership of data points as defined in~\cref{sec:generic-provenance-layer}. Since data point ownership is the decisive factor with regard to who can create provenance records for which particular data points, contracts in the specific provenance layer are responsible for actually assigning ownership, i.e., they define which clients become the owners of which data points, or rather in the notion of tokens, which tokens get assigned to which clients. For simplicity, our prototype automatically assigns new tokens to requesting clients. However, ultimately, the most suitable approach is dictated by the specific use case at hand. Two possible alternative strategies for assigning ownership are listed below:

\begin{itemize}[leftmargin=*]
	\item One possibility is for clients to purchase tokens. This has the advantage that the framework is publicly available without the risk of spamming attacks since the acquisition of tokens incurs financial cost.
	Essentially, the token acquisition costs need to be low enough for honest users to be willing and able to participate, but high enough to discourage spammers. Of course, such an approach cannot prevent malicious actors with sufficient purchasing power.
	\item In another approach, the layer manages a white list of authorised clients allowed to request new tokens. This way, the list controls exactly who participates in the provenance system. However, the question arises who is responsible for managing the white list of authorised clients.
	%\item Yet another approach is a list of pending requests. A client sends a transaction requesting tokens. An administrator gets notified about the new request and decides whether to accept or deny the request by assigning or not assigning corresponding tokens. While this approach allows a more fine-grained control over whose requests get accepted and whose requests get denied, it bears the risk of a high degree of centralisation due to the administrator having full control over distributing tokens.
\end{itemize}

%i.e., defining the notion of \emph{context} so that it reflects the provenance information needed for the specific use case. For instance, a contract could define their own function for creating provenance records. The parameters of this function are then combined to form the context field which is passed to the . \todo{Ich bin mir nicht sicher ob hier ausreichend klar wird was Beispiele solcher speziellen Informationen sind. Eventuell ein kurzes Beispiel bringen (es reicht ein kurzer Halbsatz)?}





==> sections/04scalability.tex <==
\section{Scalable Data Provenance}
\label{sec:scalability}
%So far, we have looked at how we can utilise the data provenance model from \cref{sec:provenance-model} to satisfy the functional requirements of the provenance system. By leveraging blockchain technology, we can also fulfil the non-functional requirement of providing strong integrity guarantees. We do this by breaking up the functionality of the provenance system into several abstraction layers which reside within a smart contract platform. 

%As stated above, guaranteeing integrity is crucial in provenance systems. Without integrity, data can become subject to repudiation and becomes practically worthless. Since blockchain technology provides strong integrity guarantees without the need to trust a third-party it builds the base layer for our framework. 

%However, this choice comes with a couple of downsides. Blockchains are transparent and highly inefficient in nature. While transparency does provide availability (i.e., participants can verify the integrity of the data), it also means that data on the blockchain cannot be easily hidden from unauthorised parties which breaks confidentiality/privacy. Further, computations on the blockchain are slow and expensive. This breaks the requirement for efficiency/scalability which can be especially crucial for IoT applications~[\hlr{citation?}].

The fundamental design of what makes the blockchain so secure, causes its limited scalability~\cite{christidis2016blockchains}. Thus, merely packaging a data provenance model within a smart contract platform is not enough for providing a provenance framework that is useful for IoT scenarios, since the IoT potentially involves hardware-constrained devices, frequent data updates, and massive amounts of data~\cite{fernandez2018review}. Following, we review some of the various blockchain scalability solutions with regard to their suitability as scalability solutions in an IoT data provenance framework. 

%In the following sections, we describe the scalability problem of blockchains and analyse some of the various solutions looking to overcome this issue. Finally, we make the case for so-called \emph{sidechains}~\cite{back2014enabling} as well-suited scalability solution for a blockchain-based provenance system for the IoT.

%\subsection{The Scalability Problem}
%\label{sec:scalability-problem}
%As has shortly been already addressed in \cref{cha:background}, scalability is a pressing issue of blockchain technology, especially for public blockchains like Bitcoin and Ethereum~\cite{yli2016current}. As we have seen, a public blockchain that uses PoW as its consensus protocol is primarily secured by the overall computing power within the network and its number of participants. The more computing power lies within the network, the more computing power is needed by an adversary to game the system with so-called 51\% attacks. It is further desirable to have that computing power distributed among many participants since few participants yield the risk of centralisation and consequently opportunities for abuse. The more participants, the better.

%Besides consuming computational resources to solve the PoW puzzle in order to append new blocks to the blockchain, an essential task of each participant is to make sure that no invalid blocks get added in the first place. Whenever a miner claims to have mined a new block, all other participants validate the block to decide whether to accept or reject it as the new state of the truth. Checking the validity of a block is done by repeating all steps of building the block. That means, each and every transaction that went into building the block has to be replayed by the verifier. Clearly, the more transactions a block contains, the longer it takes and the more resources are required to verify its validity. Thus, to keep the time to validate blocks relatively constant, blockchains like Bitcoin and Ethereum limit the number of transactions that can be included with each block. 

%Bitcoin does this by limiting the block size to 1 megabyte (1,000,000 bytes)~\cite{bitcoin2017wiki-scalability-faq}. With a block confirmation rate of about 600 seconds and an average transaction size of about 250 bytes, this leads to a rate of transactions per second (TPS) of about:

%\begin{displaymath}
%	1000000~\si{bytes}~/~250~\si{bytes}~/~600~\si{seconds} \approx 6,7~\si{TPS}
%\end{displaymath}

%Ethereum limits the number of transactions in a slightly different way. Instead of limiting the block size, Ethereum enforces a maximum gas limit for each block~\cite{wood2014ethereum}. As explained in \cref{cha:background}, each transaction in Ethereum costs a certain amount of gas. The total amount of gas consumed by all transactions in a block may not exceed the block's gas limit, thus effectively limiting the number of transactions that can be included in a block. The gas limit is not fixed like in Bitcoin and can be adjusted by each miner for each block by a certain amount. At the time of writing (Block 6,428,040) the gas limit is 8,000,029 gas~\cite{block6428040}. With a block gas limit of 8,000,029 gas, the minimum gas cost of a transaction of 21,000 gas and a block validation time of roughly 15 seconds, this leads to a potential throughput of about:

%\begin{displaymath}
%	8000029~\si{gas}~/~21000~\si{gas}~/~15~\si{seconds} \approx 25~\si{TPS}
%\end{displaymath}

%With an increasing number of transactions within the network, transactions have to compete with each other to be included and processed within the next block. In Bitcoin, this means a higher transaction fee has to be paid, while in Ethereum, the gas price increases. In short, transaction confirmations become slower and more expensive. Increasing the number of miners cannot increase transaction throughput since each miner has to process each and every transaction~\cite{buterin2013ethereum}. Thus, the fundamental design of what makes the blockchain so secure, is what hinders its scalability~\cite{christidis2016blockchains}.

%Besides transactions becoming slower and more expensive as the number of transactions increases, the total size of the blockchain increases as well, due to data and computation on blockchains being fully replicated in the peer-to-peer network~\cite{eberhardt2017or}. At the time of writing\footnote{30 September 2018}, the size of the Bitcoin blockchain exceeds 180 gigabyte (GB)~\cite{bitcoin2018blockchainsize}. Ethereum's blockchain even exceeds 1 terabyte (TB)~\cite{ethereum2018blockchainsize}.
%\\\\
%Expensive transactions and slow confirmation times as well as an ever increasing blockchain size pose an issue when evaluating possible use cases for blockchain technology in IoT scenarios. IoT applications are characterised by a huge number of participating nodes with scarce computational resources~\cite{atzori2010internet}. Consequently, the blockchain size prevents nodes from becoming full participants in a blockchain network. Further, IoT applications produce massive amounts of data characterised by frequent data updates (e.g., sensor value updates)~\cite{al2015internet}. When trying to take advantage of the blockchain's security properties, these massive amounts of data and frequent data updates, may pose an unsurmountable burden, because of the expensive data storage and computation within blockchains. Hence, the current state of blockchain scalability prevents IoT applications from taking full advantage of the blockchain's intrinsic security properties. However, because scalability is such a pressing issue in the blockchain space, a number of proposed solutions are underway trying to overcome these issues. Next, we address some of these solutions and examine which ones may be suitable to be adopted in a data provenance solution for the IoT.

\subsection{Scalability Solutions}
\label{sec:scalability-solutions}
Scalability solutions can generally be divided into ``layer~1'' solutions and ``layer~2'' solutions~\cite{bitcoin2017wiki-scalability-faq}. Layer 1 solutions regard the base layer of the blockchain. They seek to make improvements to the underlying protocols of the blockchain to improve its overall scalability. Some proposed solutions for improving layer 1 scalability are raising the block size limit and sharding. Contrary to layer 1 scalability solutions, layer 2 scalability solutions are not rooted at the base layer and generally revolve around the question of which data and computation should be performed \emph{on} the blockchain versus which data and computation should be performed \emph{off} the blockchain~\cite{eberhardt2017or}. Examples for layer~2 solutions are state channels~\cite{eberhardt2017or}, zero-knowledge proofs~\cite{eberhardt2018zokrates}, and sidechains~\cite{back2014enabling}.

%A number of solutions are in development trying to overcome the scalability issues of blockchain technology. Generally, these solutions can be divided into ``layer~1'' solutions and ``layer~2'' solutions~\cite{bitcoin2017wiki-scalability-faq}. Layer 1 solutions regard the base layer of the blockchain. They seek to make improvements to the underlying protocols of the blockchain to improve its overall scalability. Some proposed solutions for improving layer 1 scalability are raising the block size limit and sharding. On the contrary, layer~2 scalability solutions do not regard the base layer of the blockchain, they do not aim to improve the general scalability of the blockchain. Rather, they try to implement protocols built on top of the base layer which enable higher scalability for specific use cases. Examples for layer~2 solutions are state channels, zkSNARKs, and sidechains.

%\subsubsection{Layer 1 Scalability}
%\label{sec:layer1scalability}
%As stated above, layer 1 scalability solutions address the base layer of the blockchain. That means, these solutions are concerned with making improvements to the fundamental protocols of the blockchain in order to make it faster for all applications and services running on top of it. We can think about layer 1 scalability in two ways: horizontal scalability and vertical scalability. Horizontal scalability means ``scaling out horizontally''. What that usually refers to is adding more nodes to an existing distributed system in order to distribute the work load evenly among all nodes. Vertical scalability by contrast refers to increasing the capabilities of an existing node. That means, after scaling vertically the individual node is able to take on more work than before. 

%In terms of blockchains, horizontal scalability poses a problem. As explained in \cref{sec:scalability-problem}, each participant in a blockchain network has to process each and every transaction. This property is what makes blockchains so secure on the one hand, but so slow on the other. Thus, adding more nodes to the network does not scale the blockchain since all nodes, old and new, still have to process all transactions. Thus, often the only way to scale the base layer of a blockchain network is to undertake vertical scaling. Raising the block size limit is such a vertical scaling technique.

\subsubsection{Raising the block size limit}
Raising the block size limit is an obvious but problematic solution for improving blockchain scalability. The block size limit is used to limit the number of transactions that can be included within each block. A raised block size limit in theory allows for more transactions to be included within each block thus increasing throughput.  

%Raising the block size limit is one solution for increasing transaction throughput. As explained in \cref{sec:scalability-problem}, the block size limit is used to limit the number of transactions that can be included within each block. If the number of transactions is limited, the computational resources required to validate a block remain constant. That means, more nodes can actively participate in the validation process increasing the security of the blockchain. However, the block size limit is the primary reason why the transaction throughput of many blockchain networks is so low, e.g., $\sim$6,7~TPS and $\sim$25~TPS in the cases of Bitcoin and Ethereum, respectively. Thus, an obvious solution to increase the transaction throughput is to raise the block size limit or increase the gas limit, respectively. And in fact, raising the block size limit has been an ongoing discussion in the Bitcoin community~\cite{bitcoin2017wiki-scalability-faq} and the average gas limit has already been increased several times in the history of Ethereum~(see \cref{fig:chart-gaslimit}).

However, doing so promotes centralisation. As the size of each block grows, validator nodes have to process more and more data, therefore raising the hardware requirements for each validator. In consequence, some nodes will no longer be able to act as validators because they do not possess the necessary hardware. Thus, scaling vertically by increasing block size reduces the decentralisation of the network---one of the pillars on which the security model of blockchains is built. These shortcomings are also relevant for blockchain applications targeting the IoT. A blockchain where hardware requirements are so high that only supercomputers are able to run full validator nodes is not suitable for the IoT, since IoT applications are usually characterised by devices with low computational resources~\cite{baracaldo2017securing}.

%The major objection about raising the block size limit is that doing so promotes centralisation. As the size of each block grows, validator nodes have to process more and more data, therefore raising the hardware requirements for each validator. In consequence, some nodes will not be able to act as validators anymore because they do not possess the necessary hardware. Carrying this too far, only supercomputers will be able to act as validators, having absolute authority on which blocks are considered valid and which are not~\cite{ethereum2018sharding-faq}. Thus, scaling vertically by increasing block size reduces the decentralisation of the network –– one of the pillars on which the security model of blockchains is built.

%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth]{chart-gaslimit}
%	\caption{Ethereum Average Gas Limit Chart~\cite{ethereum2018gaslimitchart}}
%	\label{fig:chart-gaslimit}
%\end{figure}

\subsubsection{Sharding}
Sharding is a proposed scaling solution for the base layer of the Ethereum blockchain~\cite{ethereum2018sharding-faq}. Currently, all nodes of the blockchain are required to store the complete state, i.e., all account balances, contract code and storage, etc. They are responsible for processing and validating all transactions occurring within the network. This is what makes the blockchain very secure, but at the same time extremely slow (and expensive). 

Sharding splits the state into multiple different partitions, so-called ``shards''. The aim is to only have a subset of nodes validating each shard. If a validator only validates the transactions arriving at a specific shard, requirements for individual nodes can remain fairly low while the overall throughput of the network increases. Of course, it has to be guaranteed that the number of nodes validating each shard is still sufficiently large to keep the overall security of the network at a high level~\cite{ethereum2018sharding-faq}.

Sharding in blockchains is still under active development, so it remains an open question whether this technique can provide secure blockchain scalability at the base layer. Until then, several technological challenges need to be solved, e.g., validators taking over single shards in 51\% attacks, or ``cross-shard'' communication of smart contracts~\cite{ethereum2018sharding-faq}.

% For instance, one of these issues is validators trying to take over a single shard. In a blockchain with a PoW consensus protocol, taking over the entire network is extremely hard because it requires more than half of the entire computing power of the network~(i.e., 51\% attacks). However, in a ``sharded'' network, nodes might have enough computing power to dominate individual shards. Another problem is ``cross-shard'' communication, e.g., how contracts residing in different shards can communicate together. 

%Because of the number of open issues, scepticism remains whether or not sharding can actually provide real scalability at the base layer without sacrificing Ethereum's level of decentralisation and security~\cite{stopanddecrypt2018sharding}.

%Sharding, on the other hand, does have potential for providing scalability for blockchains at the base layer. But the technology is still in its early stages of its development facing some difficult challenges along the way. Thus, only time will tell if sharding will be able to fulfil its potential.

\subsubsection{State Channels}
State channels increase scalability by off-chaining state transitions~\cite{eberhardt2017or}. Two participants can open a state channel by locking some state on the blockchain~(e.g., in a smart contract). Once locked, they can perform any number of transactions on that state off-chain. The only requirement is that both participants sign off these transactions, using signatures verifiable on-chain, and that the transactions are ordered. This allows both participants to finalise the state on the blockchain at any time, since they can prove via the signatures that the counterpart agreed to the update. A state channel reduces the cost of transactions or hides them from outsiders since the guarantee of settling a transaction at any point is as good as having the transaction executed directly on the blockchain and only the final state update becomes visible in the blockchain~\cite{eberhardt2017or}. 

%Using state channels, state updates can now be performed securely off-chain, as the guarantee to be able to settle a transaction at any point, is almost as good as having the transaction executed directly on the blockchain~\cite{eberhardt2017or}. This leads to cost-savings in transaction fees as well as increased privacy since only the final state update becomes visible in the blockchain.

These characteristics make state channels a viable choice for increasing scalability in blockchain-based IoT applications, e.g., in scenarios with micro-transactions occurring between devices. However, the technology does have its drawbacks, too. For instance, state channels can only have two participants. If other users are also interested in the state updates occurring between these two users, state channels are not a suitable choice.

\emph{State channels} are already in widespread use. The lightning network~\cite{lightning} offers payment channels for the Bitcoin ecosystem. For the Ethereum network, the Whisper Protocol~\cite{whisper} and Raiden~\cite{raiden} are available.

%Though the concept is quite simple, its implementation is nonetheless tricky. Not only is an extra peer-to-peer communication channel required to exchange off-chain transactions, but participants also have to stay ``online'' at all times, since malicious peers could attempt to suppress more recent transactions. If other participants are offline and thus unable to submit the newer transactions to challenge the malicious peer, the illegal state update might get finalised.


\subsubsection{Zero-knowledge proofs}
Zero-knowledge proofs are an off-chaining pattern, where a \emph{prover} tries to convince a \emph{verifier} about the correct execution of a computation without revealing the parameters of the computation to the verifier~\cite{eberhardt2017or}. The aim is for the verifier to be able to verify that the prover knows all the required input to correctly execute the computation without knowing any of the inputs herself, thus having \emph{zero-knowledge}.

To take advantage of zero-knowledge proofs in blockchains, zkSNARKs (zero-knowledge Succinct Non-interactive ARguments of Knowledge) can be employed~\cite{eberhardt2018zokrates}. This serves two purposes: resource-intensive computations can be performed off-chain; the input of computations can be kept private.

However, proof construction in zkSNARKs is computationally expensive, leading to high hardware requirements for the prover. This can be a problem in IoT scenarios when the prover is hardware-constrained. Also, off-chaining state transitions is only beneficial when the verification of the computation is less expensive than the computation itself. Thus, while zkSNARKs can greatly improve scalability and privacy, in IoT applications with many frequent but small updates (e.g., sensor value updates), the initial overhead in setting up zkSNARKs may not be cost-efficient.

%(i) Using zkSNARKS, verifiers can verify the correctness of some computation. Thus, the computation can actually be delegated to a non-trusted third-party and does not have to be performed on the blockchain. Provided that the verification of the proof is computationally less expensive than the computation itself, transaction fees can be saved. (ii) Zero-knowledge proofs require zero knowledge about the input parameters of a computation while still being able to verify the correct computation. Thus, input parameters can be kept secret by the prover and do not have to be revealed to the verifier. Traditionally in blockchains, all data is public and transparent to all participants of the network. With zero-knowledge proofs, some data does not have to be kept on the blockchain anymore, hence improving privacy.

%While the underlying cryptographic principles of zkSNARKs are highly complex, there are ongoing efforts to make zkSNARKs more accessible to developers in order to foster its adoption as a scalability and privacy-preserving solution in the blockchain ecosystem~\cite{eberhardt2018zokrates}. ZoKrates\cite{eberhardt2018zokrates} is a prime example of these efforts, offering an extensive toolbox for constructing and verifying zkSNARKs. Though the theoretical foundations of ZoKrates are blockchain-agnostic, its proof-of-concept implementation is currently adopted for the Ethereum blockchain.


\subsubsection{Sidechains}
Sidechains as introduced by~\cite{back2014enabling}, represent a layer 2 scalability solution. The main idea of sidechains is to take load off of an existing blockchain (i.e., the parent chain) by outsourcing some of its data and computation to a separate blockchain (i.e., the sidechain).

Sidechains are ``pegged'' to the parent chain, i.e., the state of the sidechain is secured via regular commits to the parent chain. Each commit to the parent chain entails the root hash of a merkle tree consisting of all transactions that have occurred on the sidechain. This way, all transactions of the sidechain are secured via a single hash on the parent chain. This link enables participants to retreat back to the secure and reliable parent chain via so-called exit transactions in case malicious behaviour is detected on the sidechain~\cite{back2014enabling}, e.g., when sidechain validators mine invalid blocks or withhold blocks completely.

While different sidechains may deploy different, more efficient consensus protocols, or have shorter block confirmation times so that transaction throughput can be increased at the base layer, scalability gains primarily stem from the fact that participants of a sidechain do not have to validate all global transactions of the parent chain anymore, but only the transactions occurring on the sidechain. Thus, a validator's hardware requirements can remain the same, while transaction throughput can be increased as transactions and data of the parent chain are split up into multiple different sidechains. As such, sidechains improve throughput rather than latency~\cite{konstantopoulos2018plasma}. Throughput can be increased even further by creating sidechains of sidechains~\cite{plasma}.

While sidechains underly the same security-scalability trade-off as any blockchain, their flexibility combined with the security of the parent chain makes them well suited for applications which do not have the same strict security requirements as cryptocurrencies like Bitcoin and Ether, but rather rely on better scalability. Further, contrary to state channels, sidechains are fully-fledged blockchains. Hence, they can have an unlimited number of participants. At the same time, since hardware requirements for validators remain small, the entry barriers to use the system are low.

These properties make sidechains a suitable choice for global IoT scenarios which require a certain degree of integrity but are characterised by computationally restrained devices combined with frequent but relatively small data updates, such as an IoT data provenance system. There are already a number of sidechain projectsin development for both the Bitcoin and the Ethereum blockchains. For instance, in the Bitcoin ecosystem, the RSK project~\cite{rsk} is implementing a sidechain which will allow for the development of Turing-complete smart contracts in a similar way to Ethereum. For Ethereum, Plasma~\cite{plasma} and POA~\cite{poa} are available. The following section describes the data provenance solution for the IoT enhanced with sidechain technology. 



%Participants simply join a sidechain via smart contracts living on the parent chain. Sidechains improve throughput while hardware requirements for validators remain small, the entry barriers to use the system are low. 

%The general principle of sidechains can be described as follows. A participant, Alice, locks some of her funds on the parent chain via a smart contract. She then provides a proof to the sidechain that she has indeed locked some of her funds on the parent chain. The sidechain verifies the proof and if successful creates the equivalent amount of funds on the sidechain. At this point, Alice can use the funds on the sidechain in whichever way she wants, e.g., interacting with the sidechain's smart contracts, transferring funds to other participants, etc. At the end, when Alice decides to leave the sidechain, she again locks her remaining funds –– this time on the sidechain –– providing a proof that she still is the owner of the remaining funds. After the funds are locked on the sidechain, the equivalent amount of funds is released from the smart contract on the parent chain.

%Throughput can be increased even further by creating sidechains of sidechains. The overall throughput gains in a multi-level sidechain-enhanced system can roughly be calculated like this:
%
%\begin{displaymath}
%\begin{aligned}
%	{Throughput} ={} & {sidechain~throughput}\\
%					 & * {no.~sidechains~per~layer}^{no.~sidechain~layers}
%\end{aligned}
%\end{displaymath}
%
%If we assume that transaction throughput of each sidechain is about 10 TPS and each chain has three pegged sidechains, then at level three we already have a transaction throughput of $10*3^2 = 90$ TPS. At six and twelve layers we reach transaction throughputs of $10*3^5 = 2430$ TPS and $10*3^{11} = 1,78$ mio TPS, respectively. Security is maintained because each participant watches not only the chains they use, but also the links up to the parent chain for any malicious behaviour. In case any fraud is detected, they can object and retreat back to the parent chain.



\subsection{Scalable Data Provenance Using Sidechains}
\label{sec:scalable-provenance}
The essence of the framework lies in the creation of provenance records for data points. The ownership of a particular token allows participants to create provenance records for the associated data point. Thus, it is crucial that the access to tokens is strictly protected. We therefore demand clients of the provenance system to acquire tokens via a smart contract on the parent chain. This way, the system controls who acquires tokens using the security of the parent chain.

%Like any Plasma-based system, the solution consists of a Plasma contract on the parent chain and Plasma sidechains. The essence of the data provenance system lies in the creation of provenance records for data points. In ~\cref{sec:design-ownership}, we talked about the concept of ownership of data points and how ownership is represented by tokens. The ownership of a particular token allows participants to create provenance records for the associated data point. Thus, it is crucial that tokens cannot get in the hands of malicious actors and that malicious actors cannot create tokens out of thin air. The assignment and transfer of tokens have to underly strict security guarantees. We therefore demand clients of the provenance system to acquire tokens via the Plasma contract on the parent chain. This way, the system controls who acquires tokens using the security of the parent chain.

Once the system has assigned tokens to clients, these clients need to create a potentially very large number of provenance records. Because token ownership is protected via the parent chain, clients can move tokens freely onto different sidechains. Each chain can represent different IoT provenance use cases~(\cref{fig:provenance-sidechains}). For example, there might be a sidechain representing the provenance system of a vaccine supply chain as described in~\cref{sec:background}. Another chain might implement a provenance use case in a smart manufacturing scenario, etc. Each of these chains apply their own security-scalability trade-offs using different consensus protocols and network topologies depending on the requirements of the use case at hand, however in case trust in one of the sidechains is eroded or malicious behaviour is detected, clients can always retreat back to the parent chain.

\begin{figure}
	\centering
	\includegraphics[width=0.49\textwidth]{provenance-sidechains}
	\caption{Data Provenance Sidechain Architecture}
	\label{fig:provenance-sidechains}
\end{figure}

%\hlr{(}For instance, in the vaccine supply chain provenance scenario, the WHO may run a sidechain on which clients can create provenance records. Because tokens can always be withdrawn from the sidechain, even though the WHO is highly trusted, clients participating in the provenance system are not dependent on the WHO. In case trust in the WHO is eroded or clients do not wish to participate any more, they simply retreat back to the parent chain without having their tokens in jeopardy. In a slightly different scenario, each part of the vaccine supply chain might be represented by different sidechains run by different operators in different countries. Here, clients move their tokens from chain to chain as their vaccines move along the supply chain. They do not have to trust each operator, as the link back to the parent chain gives them the guarantee that their tokens cannot be stolen and that tokens cannot be created out of thin air. The only requirement is that clients observe the chains they have a stake in, and, in case malicious behaviour is detected, challenge the block or exit the chain entirely.\hlr{) - remove paragraph?}

%\subsubsection{Plasma}
%As explained above, sidechains manage their own network topology, consensus protocol, etc. They are therefore not classified as technology per se, but more as a design pattern which can be used to derive architectures for application-specific sidechains. 

%Though the described sidechain-enhanced data provenance solution for the IoT is blockchain agnostic, we illustrate sidechain architecture of the solution based on Plasma~\cite{plasma} –– a sidechain paradigm available for the Ethereum blockchain. Plasma consists of the following components: a Plasma (side)chain, and a Plasma (smart) contract deployed on the parent chain (Ethereum).

%\begin{figure}[!b]
%	\centering
%	\includegraphics[width=11cm]{plasma-1}
%	\caption{Joining a Plasma Chain}
%	\label{fig:plasma-1}
%\end{figure}

%The general concept of Plasma can be explained as follows. A participant –– Alice –– decides she wants to participate in a Plasma chain. She joins the Plasma chain by sending a transaction to the Plasma contract on the parent chain locking some of her funds represented by tokens. Once the transaction is processed, the Plasma contract emits a ``Deposit'' event. The event is picked up by the listening Plasma chain which immediately creates the same amount of tokens for Alice on the Plasma chain~(\cref{fig:plasma-1}).

%\begin{figure}
%	\centering
%	\includegraphics[width=11cm]{plasma-2}
%	\caption{Executing Transactions on the Plasma Chain}
%	\label{fig:plasma-2}
%\end{figure}

%Alice can now use these tokens on the Plasma chain, e.g., she might create a transaction transferring a certain amount of tokens to Bob. These transactions are included in blocks in the Plasma chain, but they are not finalised yet. In regular intervals, the hashes of the blocks of the Plasma chain are committed to the parent chain. Once the block hash is committed and after a certain \emph{challenge period} has passed, the contained transactions are finalised~(\cref{fig:plasma-2}). This greatly reduces storage requirements for the parent chain as storing the block hash costs only a minimal amount in comparison to storing all transactions. This is where the main scalability gains are made. Alice still has to wait for her transactions to be committed to the parent chain, but because the actual transactions are processed and stored on the Plasma chain, transaction throughput increases.

%\begin{figure}[!b]
%	\centering
%	\includegraphics[width=11cm]{plasma-3}
%	\caption{Redeeming Funds on the Parent Chain}
%	\label{fig:plasma-3}
%\end{figure}

%After a while, Alice may decide to leave the Plasma chain. She therefore sends a transaction to the Plasma chain saying she wants to move her funds back to the parent chain. Once the most recent block hash is included in the parent chain, and after a challenge period has passed, her funds are released again~(\cref{fig:plasma-3}).

%\paragraph{Detecting Fraud} \hfill \\
%Because only the block hashes of the Plasma chain are stored in the parent chain, transactions happening on the Plasma chain cannot be validated by parent chain validators. Instead, participants of a Plasma chain have to make sure no invalid block hashes are committed to the parent chain in order to avoid fraud. Basically, two main fraud scenarios exist:
%\pagebreak
%\begin{enumerate}
%	\item Someone trying to execute invalid state transitions (e.g., stealing someone's funds).
%	\item Someone trying to create tokens out of thin air.
%\end{enumerate}
%
%The first case can be prevented by having participants of the Plasma chain ``watch'' the Plasma chain as well as the link to the parent chain for any malicious behaviour. For example, the Plasma operator might try to steal the tokens of Alice by appending a forged block to the Plasma chain. When Alice detects such an invalid block, she can challenge it by providing a proof that the block is invalid. If the challenge is successful, Alice wins a stake from the Plasma operator and the corresponding block is rolled back. In fact, winning the stake is an incentive for any participant to challenge such an illegal block. In another scenario, the Plasma operator could try to withhold the invalid block from the other participants. In such a case of data unavailability, Plasma provides the mechanism of so-called \emph{exits}: participants detect that a block hash was committed to the parent chain without being able to see the corresponding data. In this case, participants can send an exit transaction within the challenge period which withdraws their funds back to the parent chain.
%
%In the second case, someone tries to create tokens in a Plasma chain out of thin air and then tries to move these tokens back to the parent chain. To mitigate this, Plasma keeps track of the number of tokens that were transferred to a Plasma chain. The rule is that not more tokens can be withdrawn from a Plasma chain than were deposited in the first place. Thus, it is not possible to create tokens out of thin air.
%
%We see that Plasma provides the possibility to take load off of the parent chain by ``off-chaining'' certain data and transactions to a separate blockchain without abandoning the security guarantees of the parent chain.





==> sections/05discussion.tex <==
\section{Discussion}
\label{sec:discussion}
As we have demonstrated, the presented framework is able to satisfy~\Crefrange{req:abstraction}{req:parallel} by building on top of the generic data provenance model for the IoT and by providing abstraction layers which specific use cases can adopt to their own requirements such as the assignment of ownership of data point IDs. Further, the framework relies on blockchain technology to provide guarantees of integrity and availability~(\Cref{req:integrity} and \Cref{req:availability}). However, the fundamental design of what makes the blockchain secure causes its limited scalability and privacy~\cite{christidis2016blockchains}. While in some cases a private blockchain can be employed to provide better privacy and scalability~\cite{griggs2018healthcare}, in global IoT scenarios entailing massive amounts of data and frequent data updates where public access to the system is necessary, a private blockchain might not be a viable option~\cite{fernandez2018review}. Hence, a solution is needed to improve the privacy and scalability properties of a public blockchain system while keeping its integrity and availability guarantees. Several recent blockchain developments try to tackle these limitations, e.g., state channels~\cite{eberhardt2017or}, zero-knowledge proofs~\cite{eberhardt2018zokrates}, and sidechains~\cite{back2014enabling}. %In the following, we discuss recent blockchain developments with respect to their suitability in a data provenance solution for the IoT.

%\hlr{(}Blockchain developments that attempt to solve the blockchain's inherent privacy and scalability issues can generally be divided into ``layer~1'' and ``layer~2'' solutions~\cite{bitcoin2017wiki-scalability-faq}. ``Layer 1'' solutions regard the base layer of the blockchain. They seek to make improvements to the underlying protocols of the blockchain. Some proposed ``layer~1'' solutions are raising the block size limit and sharding. Contrary to ``layer 1'' solutions, ``layer 2'' solutions are not rooted at the base layer and generally revolve around the question of which data and computation should be performed on the blockchain versus which data and computation should be performed off the blockchain~\cite{eberhardt2017or}. Examples for ``layer~2'' solutions are state channels~\cite{eberhardt2017or}, zero-knowledge proofs~\cite{eberhardt2018zokrates}, and sidechains~\cite{back2014enabling}. In the following, we look at some of these approaches with regards to their suitability in a data provenance solution for the IoT.\hlr{)}

%For instance, a specific provenance contract could limit the number of characters of the context string. If the context string gets too big to store all necessary provenance information, clients could store the context in a content-addressable storage such as the Interplanetary File System~(IPFS\footnote{\url{https://ipfs.io/}}) and store the content's hash sum as context parameter of a new provenance record within the system. This would enable the storage of large amounts of provenance information while keeping storage costs relatively low. Since gas consumption rises even more rapidly when increasing the number of input provenance records, this parameter should also be limited by specific provenance contracts. Here, it is important to estimate the potential number of input provenance records within the concrete use case and implement the limit accordingly.

%So far, we have looked at how we can utilise the data provenance model from \cref{sec:provenance-model} to satisfy the functional requirements of the provenance system. By leveraging blockchain technology, we can also fulfil the non-functional requirement of providing strong integrity guarantees. We do this by breaking up the functionality of the provenance system into several abstraction layers which reside within a smart contract platform. 

%As stated above, guaranteeing integrity is crucial in provenance systems. Without integrity, data can become subject to repudiation and becomes practically worthless. Since blockchain technology provides strong integrity guarantees without the need to trust a third-party it builds the base layer for our framework. 

%However, this choice comes with a couple of downsides. Blockchains are transparent and highly inefficient in nature. While transparency does provide availability (i.e., participants can verify the integrity of the data), it also means that data on the blockchain cannot be easily hidden from unauthorised parties which breaks confidentiality/privacy. Further, computations on the blockchain are slow and expensive. This breaks the requirement for efficiency/scalability which can be especially crucial for IoT applications~[\hlr{citation?}].

 %Thus, merely packaging a data provenance model within a smart contract platform is not enough for providing a provenance framework that is useful for IoT scenarios, since the IoT potentially involves hardware-constrained devices, frequent data updates, and massive amounts of data~\cite{fernandez2018review}. Following, we review some of the various blockchain scalability solutions with regard to their suitability as scalability solutions in an IoT data provenance framework. 

%In the following sections, we describe the scalability problem of blockchains and analyse some of the various solutions looking to overcome this issue. Finally, we make the case for so-called \emph{sidechains}~\cite{back2014enabling} as well-suited scalability solution for a blockchain-based provenance system for the IoT.

%\subsection{The Scalability Problem}
%\label{sec:scalability-problem}
%As has shortly been already addressed in \cref{cha:background}, scalability is a pressing issue of blockchain technology, especially for public blockchains like Bitcoin and Ethereum~\cite{yli2016current}. As we have seen, a public blockchain that uses PoW as its consensus protocol is primarily secured by the overall computing power within the network and its number of participants. The more computing power lies within the network, the more computing power is needed by an adversary to game the system with so-called 51\% attacks. It is further desirable to have that computing power distributed among many participants since few participants yield the risk of centralisation and consequently opportunities for abuse. The more participants, the better.

%Besides consuming computational resources to solve the PoW puzzle in order to append new blocks to the blockchain, an essential task of each participant is to make sure that no invalid blocks get added in the first place. Whenever a miner claims to have mined a new block, all other participants validate the block to decide whether to accept or reject it as the new state of the truth. Checking the validity of a block is done by repeating all steps of building the block. That means, each and every transaction that went into building the block has to be replayed by the verifier. Clearly, the more transactions a block contains, the longer it takes and the more resources are required to verify its validity. Thus, to keep the time to validate blocks relatively constant, blockchains like Bitcoin and Ethereum limit the number of transactions that can be included with each block. 

%Bitcoin does this by limiting the block size to 1 megabyte (1,000,000 bytes)~\cite{bitcoin2017wiki-scalability-faq}. With a block confirmation rate of about 600 seconds and an average transaction size of about 250 bytes, this leads to a rate of transactions per second (TPS) of about:

%\begin{displaymath}
%	1000000~\si{bytes}~/~250~\si{bytes}~/~600~\si{seconds} \approx 6,7~\si{TPS}
%\end{displaymath}

%Ethereum limits the number of transactions in a slightly different way. Instead of limiting the block size, Ethereum enforces a maximum gas limit for each block~\cite{wood2014ethereum}. As explained in \cref{cha:background}, each transaction in Ethereum costs a certain amount of gas. The total amount of gas consumed by all transactions in a block may not exceed the block's gas limit, thus effectively limiting the number of transactions that can be included in a block. The gas limit is not fixed like in Bitcoin and can be adjusted by each miner for each block by a certain amount. At the time of writing (Block 6,428,040) the gas limit is 8,000,029 gas~\cite{block6428040}. With a block gas limit of 8,000,029 gas, the minimum gas cost of a transaction of 21,000 gas and a block validation time of roughly 15 seconds, this leads to a potential throughput of about:

%\begin{displaymath}
%	8000029~\si{gas}~/~21000~\si{gas}~/~15~\si{seconds} \approx 25~\si{TPS}
%\end{displaymath}

%With an increasing number of transactions within the network, transactions have to compete with each other to be included and processed within the next block. In Bitcoin, this means a higher transaction fee has to be paid, while in Ethereum, the gas price increases. In short, transaction confirmations become slower and more expensive. Increasing the number of miners cannot increase transaction throughput since each miner has to process each and every transaction~\cite{buterin2013ethereum}. Thus, the fundamental design of what makes the blockchain so secure, is what hinders its scalability~\cite{christidis2016blockchains}.

%Besides transactions becoming slower and more expensive as the number of transactions increases, the total size of the blockchain increases as well, due to data and computation on blockchains being fully replicated in the peer-to-peer network~\cite{eberhardt2017or}. At the time of writing\footnote{30 September 2018}, the size of the Bitcoin blockchain exceeds 180 gigabyte (GB)~\cite{bitcoin2018blockchainsize}. Ethereum's blockchain even exceeds 1 terabyte (TB)~\cite{ethereum2018blockchainsize}.
%\\\\
%Expensive transactions and slow confirmation times as well as an ever increasing blockchain size pose an issue when evaluating possible use cases for blockchain technology in IoT scenarios. IoT applications are characterised by a huge number of participating nodes with scarce computational resources~\cite{atzori2010internet}. Consequently, the blockchain size prevents nodes from becoming full participants in a blockchain network. Further, IoT applications produce massive amounts of data characterised by frequent data updates (e.g., sensor value updates)~\cite{al2015internet}. When trying to take advantage of the blockchain's security properties, these massive amounts of data and frequent data updates, may pose an unsurmountable burden, because of the expensive data storage and computation within blockchains. Hence, the current state of blockchain scalability prevents IoT applications from taking full advantage of the blockchain's intrinsic security properties. However, because scalability is such a pressing issue in the blockchain space, a number of proposed solutions are underway trying to overcome these issues. Next, we address some of these solutions and examine which ones may be suitable to be adopted in a data provenance solution for the IoT.

%\subsection{Scalability Solutions}
%\label{sec:scalability-solutions}
%Blockchain developments that attempt to solve the blockchain's inherent privacy and scalability issues can generally be divided into ``layer~1'' and ``layer~2'' solutions~\cite{bitcoin2017wiki-scalability-faq}. Layer 1 solutions regard the base layer of the blockchain. They seek to make improvements to the underlying protocols of the blockchain. Some proposed ``layer~1'' solutions are raising the block size limit and sharding. Contrary to layer 1 solutions, layer 2 solutions are not rooted at the base layer and generally revolve around the question of which data and computation should be performed \emph{on} the blockchain versus which data and computation should be performed \emph{off} the blockchain~\cite{eberhardt2017or}. Examples for layer~2 solutions are state channels~\cite{eberhardt2017or}, zero-knowledge proofs~\cite{eberhardt2018zokrates}, and sidechains~\cite{back2014enabling}.

%Scalability solutions can generally be divided into ``layer~1'' solutions and ``layer~2'' solutions~\cite{bitcoin2017wiki-scalability-faq}. Layer 1 solutions regard the base layer of the blockchain. They seek to make improvements to the underlying protocols of the blockchain to improve its overall scalability. Some proposed solutions for improving layer 1 scalability are raising the block size limit and sharding. Contrary to layer 1 scalability solutions, layer 2 scalability solutions are not rooted at the base layer and generally revolve around the question of which data and computation should be performed \emph{on} the blockchain versus which data and computation should be performed \emph{off} the blockchain~\cite{eberhardt2017or}. Examples for layer~2 solutions are state channels~\cite{eberhardt2017or}, zero-knowledge proofs~\cite{eberhardt2018zokrates}, and sidechains~\cite{back2014enabling}.

%A number of solutions are in development trying to overcome the scalability issues of blockchain technology. Generally, these solutions can be divided into ``layer~1'' solutions and ``layer~2'' solutions~\cite{bitcoin2017wiki-scalability-faq}. Layer 1 solutions regard the base layer of the blockchain. They seek to make improvements to the underlying protocols of the blockchain to improve its overall scalability. Some proposed solutions for improving layer 1 scalability are raising the block size limit and sharding. On the contrary, layer~2 scalability solutions do not regard the base layer of the blockchain, they do not aim to improve the general scalability of the blockchain. Rather, they try to implement protocols built on top of the base layer which enable higher scalability for specific use cases. Examples for layer~2 solutions are state channels, zkSNARKs, and sidechains.

%\subsubsection{Layer 1 Scalability}
%\label{sec:layer1scalability}
%As stated above, layer 1 scalability solutions address the base layer of the blockchain. That means, these solutions are concerned with making improvements to the fundamental protocols of the blockchain in order to make it faster for all applications and services running on top of it. We can think about layer 1 scalability in two ways: horizontal scalability and vertical scalability. Horizontal scalability means ``scaling out horizontally''. What that usually refers to is adding more nodes to an existing distributed system in order to distribute the work load evenly among all nodes. Vertical scalability by contrast refers to increasing the capabilities of an existing node. That means, after scaling vertically the individual node is able to take on more work than before. 

%In terms of blockchains, horizontal scalability poses a problem. As explained in \cref{sec:scalability-problem}, each participant in a blockchain network has to process each and every transaction. This property is what makes blockchains so secure on the one hand, but so slow on the other. Thus, adding more nodes to the network does not scale the blockchain since all nodes, old and new, still have to process all transactions. Thus, often the only way to scale the base layer of a blockchain network is to undertake vertical scaling. Raising the block size limit is such a vertical scaling technique.

%\subsubsection{Raising the block size limit}
%Raising the block size limit is an obvious but problematic solution for improving blockchain scalability. The block size limit is used to limit the number of transactions that can be included within each block. A raised block size limit in theory allows for more transactions to be included within each block thus increasing throughput.  

%Raising the block size limit is one solution for increasing transaction throughput. As explained in \cref{sec:scalability-problem}, the block size limit is used to limit the number of transactions that can be included within each block. If the number of transactions is limited, the computational resources required to validate a block remain constant. That means, more nodes can actively participate in the validation process increasing the security of the blockchain. However, the block size limit is the primary reason why the transaction throughput of many blockchain networks is so low, e.g., $\sim$6,7~TPS and $\sim$25~TPS in the cases of Bitcoin and Ethereum, respectively. Thus, an obvious solution to increase the transaction throughput is to raise the block size limit or increase the gas limit, respectively. And in fact, raising the block size limit has been an ongoing discussion in the Bitcoin community~\cite{bitcoin2017wiki-scalability-faq} and the average gas limit has already been increased several times in the history of Ethereum~(see \cref{fig:chart-gaslimit}).

%However, as the size of each block grows, validator nodes have to process more and more data, effectively raising the hardware requirements for each validator. A blockchain where hardware requirements are so high that only supercomputers are able to run full validator nodes is not suitable for the IoT, since IoT applications are usually characterised by devices with low computational resources~\cite{baracaldo2017securing}. Further, raising the block size limit provides no solution for privacy.

%The major objection about raising the block size limit is that doing so promotes centralisation. As the size of each block grows, validator nodes have to process more and more data, therefore raising the hardware requirements for each validator. In consequence, some nodes will not be able to act as validators anymore because they do not possess the necessary hardware. Carrying this too far, only supercomputers will be able to act as validators, having absolute authority on which blocks are considered valid and which are not~\cite{ethereum2018sharding-faq}. Thus, scaling vertically by increasing block size reduces the decentralisation of the network –– one of the pillars on which the security model of blockchains is built.

%\begin{figure}
%	\centering
%	\includegraphics[width=\linewidth]{chart-gaslimit}
%	\caption{Ethereum Average Gas Limit Chart~\cite{ethereum2018gaslimitchart}}
%	\label{fig:chart-gaslimit}
%\end{figure}

%\subsubsection{Sharding}
%Sharding is a proposed scaling solution for the base layer of the Ethereum blockchain~\cite{ethereum2018sharding-faq}. Currently, all nodes of the blockchain are required to store and validate the complete state. This is what makes the blockchain very secure, and at the same time very slow (and expensive). 

%Sharding splits the state into multiple partitions, so-called ``shards''. The aim is to only have a subset of nodes validating each shard. If a validator only validates the transactions arriving at a specific shard, hardware requirements for nodes can remain fairly low while the overall throughput of the network increases. Of course, it has to be guaranteed that the number of nodes validating each shard is still sufficiently large to guarantee the overall security of the network~\cite{ethereum2018sharding-faq}.

%Sharding in blockchains is still under active development, so it remains an open question whether this technique can provide secure blockchain scalability and privacy at the base layer. Until then, several technological challenges need to be solved, e.g., validators taking over single shards in 51\% attacks, or ``cross-shard'' communication of smart contracts~\cite{ethereum2018sharding-faq}.

% For instance, one of these issues is validators trying to take over a single shard. In a blockchain with a PoW consensus protocol, taking over the entire network is extremely hard because it requires more than half of the entire computing power of the network~(i.e., 51\% attacks). However, in a ``sharded'' network, nodes might have enough computing power to dominate individual shards. Another problem is ``cross-shard'' communication, e.g., how contracts residing in different shards can communicate together. 

%Because of the number of open issues, scepticism remains whether or not sharding can actually provide real scalability at the base layer without sacrificing Ethereum's level of decentralisation and security~\cite{stopanddecrypt2018sharding}.

%Sharding, on the other hand, does have potential for providing scalability for blockchains at the base layer. But the technology is still in its early stages of its development facing some difficult challenges along the way. Thus, only time will tell if sharding will be able to fulfil its potential.

\subsubsection{State Channels}
State channels increase scalability by off-chaining state transitions~\cite{eberhardt2017or}. Two participants open a state channel by locking some state on the blockchain~(e.g., in a smart contract). Once locked, they perform transactions on that state off-chain. The only requirement is that both participants sign off these transactions, using signatures verifiable on-chain, and that the transactions are ordered. This allows both participants to finalise the state on the blockchain at any time, since they can prove via the signatures that the counterpart agreed to the update. A state channel reduces the cost of transactions or hides them from outsiders since the guarantee of settling a transaction at any point is as good as having the transaction executed directly on the blockchain and only the final state update becomes visible in the blockchain~\cite{eberhardt2017or}. These characteristics make state channels a viable choice for increasing scalability and improving privacy in blockchain-based IoT applications, e.g., in scenarios with micro-transactions occurring between devices.%However, eventually the final state is published on the blockchain. This could still yield a problem in scenarios that that involve highly sensitive data such as in a health monitoring system.

%Using state channels, state updates can now be performed securely off-chain, as the guarantee to be able to settle a transaction at any point, is almost as good as having the transaction executed directly on the blockchain~\cite{eberhardt2017or}. This leads to cost-savings in transaction fees as well as increased privacy since only the final state update becomes visible in the blockchain.

%These characteristics make state channels a viable choice for increasing scalability in blockchain-based IoT applications, e.g., in scenarios with micro-transactions occurring between devices. However, the technology does have its drawbacks, too. For instance, state channels can only have two participants. If other users are also interested in the state updates occurring between these two users, state channels are not a suitable choice.

%\hlr{(}\emph{State channels} are already in widespread use. The lightning network~\cite{lightning} offers payment channels for the Bitcoin ecosystem. For the Ethereum network, the Whisper Protocol~\cite{whisper} and Raiden~\cite{raiden} are available.\hlr{)}

%Though the concept is quite simple, its implementation is nonetheless tricky. Not only is an extra peer-to-peer communication channel required to exchange off-chain transactions, but participants also have to stay ``online'' at all times, since malicious peers could attempt to suppress more recent transactions. If other participants are offline and thus unable to submit the newer transactions to challenge the malicious peer, the illegal state update might get finalised.


\subsubsection{Zero-knowledge proofs}
Zero-knowledge proofs are an off-chaining pattern, where a prover tries to convince a verifier about the correct execution of a computation without revealing the parameters of the computation to the verifier~\cite{eberhardt2017or}. The aim is for the verifier to be able to verify that the prover correctly executed the computation without the verifier knowing any of the inputs required for the computation, thus having zero knowledge. To take advantage of zero-knowledge proofs in blockchains, zkSNARKs (zero-knowledge Succinct Non-interactive ARguments of Knowledge) can be employed~\cite{eberhardt2018zokrates}. This serves two purposes: resource-intensive computations can be performed and verified off-chain and the input of computations can be kept private.

However, proof construction in zkSNARKs is computationally expensive, leading to high hardware requirements for the prover. This can be a problem in IoT scenarios when the prover is hardware-constrained. Also, off-chaining state transitions is only beneficial when the verification of the computation is less expensive than the computation itself. Thus, while zkSNARKs can improve scalability and privacy, it needs to be evaluated whether the initial overhead is justifiable in IoT applications.

%(i) Using zkSNARKS, verifiers can verify the correctness of some computation. Thus, the computation can actually be delegated to a non-trusted third-party and does not have to be performed on the blockchain. Provided that the verification of the proof is computationally less expensive than the computation itself, transaction fees can be saved. (ii) Zero-knowledge proofs require zero knowledge about the input parameters of a computation while still being able to verify the correct computation. Thus, input parameters can be kept secret by the prover and do not have to be revealed to the verifier. Traditionally in blockchains, all data is public and transparent to all participants of the network. With zero-knowledge proofs, some data does not have to be kept on the blockchain anymore, hence improving privacy.

%While the underlying cryptographic principles of zkSNARKs are highly complex, there are ongoing efforts to make zkSNARKs more accessible to developers in order to foster its adoption as a scalability and privacy-preserving solution in the blockchain ecosystem~\cite{eberhardt2018zokrates}. ZoKrates\cite{eberhardt2018zokrates} is a prime example of these efforts, offering an extensive toolbox for constructing and verifying zkSNARKs. Though the theoretical foundations of ZoKrates are blockchain-agnostic, its proof-of-concept implementation is currently adopted for the Ethereum blockchain.


\subsubsection{Sidechains}
The main idea of sidechains is to take load off of an existing blockchain (i.e., the parent chain) by outsourcing some of its data and computation to a separate blockchain (i.e., the sidechain)~\cite{back2014enabling}. Sidechains are ``pegged'' to the parent chain, i.e., the state of the sidechain is secured via regular commits to the parent chain. Such commits entail the root hash of a Merkle tree consisting of all transactions that have occurred on the sidechain. This way, all transactions of the sidechain are secured via a single hash on the parent chain. This link enables participants to retreat back to the secure and reliable parent chain via so-called exits in case malicious behaviour is detected on the sidechain~\cite{back2014enabling}, e.g., when sidechain validators mine invalid blocks or withhold blocks completely. While sidechains can potentially employ different, more efficient consensus mechanisms than the parent chain, scalability gains primarily derive from participants of a sidechain not having to validate all global transactions of the parent chain anymore, but only the transactions occurring on the sidechain. Thus, a validator's hardware requirements can remain low, while transaction throughput is increased as transactions and data of the parent chain are split up into multiple different sidechains. As such, sidechains improve throughput rather than latency~\cite{konstantopoulos2018plasma}. Further, sidechains could be kept secret to improve privacy.

While the above approaches are promising with regard to improving scalability and privacy of blockchain applications, in future work, it needs to be evaluated if and how these solutions can be employed to provide scalability and privacy improvements in global IoT scenarios which require a certain degree of integrity but are characterised by computationally restrained devices combined with frequent but relatively small data updates.

%As we have seen, multiple approaches exist to overcome the privacy and scalability problems of blockchains. In future work, we will evaluate in detail to what extent these approaches provide solutions to the privacy and scalability problem in the context of blockchain-enhanced IoT applications, such as our data provenance framework. In particular, prototypes based on zero-knowledge proofs, state channels, and sidechains will be implemented and compared.

%There are already a number of sidechain projectsin development for both the Bitcoin and the Ethereum blockchains. For instance, in the Bitcoin ecosystem, the RSK project~\cite{rsk} is implementing a sidechain which will allow for the development of Turing-complete smart contracts in a similar way to Ethereum. For Ethereum, Plasma~\cite{plasma} and POA~\cite{poa} are available. The following section describes the data provenance solution for the IoT enhanced with sidechain technology. 



%Participants simply join a sidechain via smart contracts living on the parent chain. Sidechains improve throughput while hardware requirements for validators remain small, the entry barriers to use the system are low. 

%The general principle of sidechains can be described as follows. A participant, Alice, locks some of her funds on the parent chain via a smart contract. She then provides a proof to the sidechain that she has indeed locked some of her funds on the parent chain. The sidechain verifies the proof and if successful creates the equivalent amount of funds on the sidechain. At this point, Alice can use the funds on the sidechain in whichever way she wants, e.g., interacting with the sidechain's smart contracts, transferring funds to other participants, etc. At the end, when Alice decides to leave the sidechain, she again locks her remaining funds –– this time on the sidechain –– providing a proof that she still is the owner of the remaining funds. After the funds are locked on the sidechain, the equivalent amount of funds is released from the smart contract on the parent chain.

%Throughput can be increased even further by creating sidechains of sidechains. The overall throughput gains in a multi-level sidechain-enhanced system can roughly be calculated like this:
%
%\begin{displaymath}
%\begin{aligned}
%	{Throughput} ={} & {sidechain~throughput}\\
%					 & * {no.~sidechains~per~layer}^{no.~sidechain~layers}
%\end{aligned}
%\end{displaymath}
%
%If we assume that transaction throughput of each sidechain is about 10 TPS and each chain has three pegged sidechains, then at level three we already have a transaction throughput of $10*3^2 = 90$ TPS. At six and twelve layers we reach transaction throughputs of $10*3^5 = 2430$ TPS and $10*3^{11} = 1,78$ mio TPS, respectively. Security is maintained because each participant watches not only the chains they use, but also the links up to the parent chain for any malicious behaviour. In case any fraud is detected, they can object and retreat back to the parent chain.



%\subsection{Scalable Data Provenance Using Sidechains}
%\label{sec:scalable-provenance}
%The essence of the framework lies in the creation of provenance records for data points. The ownership of a particular token allows participants to create provenance records for the associated data point. Thus, it is crucial that the access to tokens is strictly protected. We therefore demand clients of the provenance system to acquire tokens via a smart contract on the parent chain. This way, the system controls who acquires tokens using the security of the parent chain.

%Like any Plasma-based system, the solution consists of a Plasma contract on the parent chain and Plasma sidechains. The essence of the data provenance system lies in the creation of provenance records for data points. In ~\cref{sec:design-ownership}, we talked about the concept of ownership of data points and how ownership is represented by tokens. The ownership of a particular token allows participants to create provenance records for the associated data point. Thus, it is crucial that tokens cannot get in the hands of malicious actors and that malicious actors cannot create tokens out of thin air. The assignment and transfer of tokens have to underly strict security guarantees. We therefore demand clients of the provenance system to acquire tokens via the Plasma contract on the parent chain. This way, the system controls who acquires tokens using the security of the parent chain.

%Once the system has assigned tokens to clients, these clients need to create a potentially very large number of provenance records. Because token ownership is protected via the parent chain, clients can move tokens freely onto different sidechains. Each chain can represent different IoT provenance use cases~(\cref{fig:provenance-sidechains}). For example, there might be a sidechain representing the provenance system of a vaccine supply chain as described in~\cref{sec:background}. Another chain might implement a provenance use case in a smart manufacturing scenario, etc. Each of these chains apply their own security-scalability trade-offs using different consensus protocols and network topologies depending on the requirements of the use case at hand, however in case trust in one of the sidechains is eroded or malicious behaviour is detected, clients can always retreat back to the parent chain.

%\begin{figure}
%	\centering
%	\includegraphics[width=0.49\textwidth]{provenance-sidechains}
%	\caption{Data Provenance Sidechain Architecture}
%	\label{fig:provenance-sidechains}
%\end{figure}

%\hlr{(}For instance, in the vaccine supply chain provenance scenario, the WHO may run a sidechain on which clients can create provenance records. Because tokens can always be withdrawn from the sidechain, even though the WHO is highly trusted, clients participating in the provenance system are not dependent on the WHO. In case trust in the WHO is eroded or clients do not wish to participate any more, they simply retreat back to the parent chain without having their tokens in jeopardy. In a slightly different scenario, each part of the vaccine supply chain might be represented by different sidechains run by different operators in different countries. Here, clients move their tokens from chain to chain as their vaccines move along the supply chain. They do not have to trust each operator, as the link back to the parent chain gives them the guarantee that their tokens cannot be stolen and that tokens cannot be created out of thin air. The only requirement is that clients observe the chains they have a stake in, and, in case malicious behaviour is detected, challenge the block or exit the chain entirely.\hlr{) - remove paragraph?}

%\subsubsection{Plasma}
%As explained above, sidechains manage their own network topology, consensus protocol, etc. They are therefore not classified as technology per se, but more as a design pattern which can be used to derive architectures for application-specific sidechains. 

%Though the described sidechain-enhanced data provenance solution for the IoT is blockchain agnostic, we illustrate sidechain architecture of the solution based on Plasma~\cite{plasma} –– a sidechain paradigm available for the Ethereum blockchain. Plasma consists of the following components: a Plasma (side)chain, and a Plasma (smart) contract deployed on the parent chain (Ethereum).

%\begin{figure}[!b]
%	\centering
%	\includegraphics[width=11cm]{plasma-1}
%	\caption{Joining a Plasma Chain}
%	\label{fig:plasma-1}
%\end{figure}

%The general concept of Plasma can be explained as follows. A participant –– Alice –– decides she wants to participate in a Plasma chain. She joins the Plasma chain by sending a transaction to the Plasma contract on the parent chain locking some of her funds represented by tokens. Once the transaction is processed, the Plasma contract emits a ``Deposit'' event. The event is picked up by the listening Plasma chain which immediately creates the same amount of tokens for Alice on the Plasma chain~(\cref{fig:plasma-1}).

%\begin{figure}
%	\centering
%	\includegraphics[width=11cm]{plasma-2}
%	\caption{Executing Transactions on the Plasma Chain}
%	\label{fig:plasma-2}
%\end{figure}

%Alice can now use these tokens on the Plasma chain, e.g., she might create a transaction transferring a certain amount of tokens to Bob. These transactions are included in blocks in the Plasma chain, but they are not finalised yet. In regular intervals, the hashes of the blocks of the Plasma chain are committed to the parent chain. Once the block hash is committed and after a certain \emph{challenge period} has passed, the contained transactions are finalised~(\cref{fig:plasma-2}). This greatly reduces storage requirements for the parent chain as storing the block hash costs only a minimal amount in comparison to storing all transactions. This is where the main scalability gains are made. Alice still has to wait for her transactions to be committed to the parent chain, but because the actual transactions are processed and stored on the Plasma chain, transaction throughput increases.

%\begin{figure}[!b]
%	\centering
%	\includegraphics[width=11cm]{plasma-3}
%	\caption{Redeeming Funds on the Parent Chain}
%	\label{fig:plasma-3}
%\end{figure}

%After a while, Alice may decide to leave the Plasma chain. She therefore sends a transaction to the Plasma chain saying she wants to move her funds back to the parent chain. Once the most recent block hash is included in the parent chain, and after a challenge period has passed, her funds are released again~(\cref{fig:plasma-3}).

%\paragraph{Detecting Fraud} \hfill \\
%Because only the block hashes of the Plasma chain are stored in the parent chain, transactions happening on the Plasma chain cannot be validated by parent chain validators. Instead, participants of a Plasma chain have to make sure no invalid block hashes are committed to the parent chain in order to avoid fraud. Basically, two main fraud scenarios exist:
%\pagebreak
%\begin{enumerate}
%	\item Someone trying to execute invalid state transitions (e.g., stealing someone's funds).
%	\item Someone trying to create tokens out of thin air.
%\end{enumerate}
%
%The first case can be prevented by having participants of the Plasma chain ``watch'' the Plasma chain as well as the link to the parent chain for any malicious behaviour. For example, the Plasma operator might try to steal the tokens of Alice by appending a forged block to the Plasma chain. When Alice detects such an invalid block, she can challenge it by providing a proof that the block is invalid. If the challenge is successful, Alice wins a stake from the Plasma operator and the corresponding block is rolled back. In fact, winning the stake is an incentive for any participant to challenge such an illegal block. In another scenario, the Plasma operator could try to withhold the invalid block from the other participants. In such a case of data unavailability, Plasma provides the mechanism of so-called \emph{exits}: participants detect that a block hash was committed to the parent chain without being able to see the corresponding data. In this case, participants can send an exit transaction within the challenge period which withdraws their funds back to the parent chain.
%
%In the second case, someone tries to create tokens in a Plasma chain out of thin air and then tries to move these tokens back to the parent chain. To mitigate this, Plasma keeps track of the number of tokens that were transferred to a Plasma chain. The rule is that not more tokens can be withdrawn from a Plasma chain than were deposited in the first place. Thus, it is not possible to create tokens out of thin air.
%
%We see that Plasma provides the possibility to take load off of the parent chain by ``off-chaining'' certain data and transactions to a separate blockchain without abandoning the security guarantees of the parent chain.




